Data Coverage for Detecting Representation Bias in Image Datasets: A Crowdsourcing Approach

Existing machine learning models have proven to fail when it comes to their performance for minority groups, mainly due to biases in data. In particular, datasets, especially social data, are often not representative of minorities. In this paper, we consider the problem of representation bias identification on image datasets without explicit attribute values. Using the notion of data coverage for detecting a lack of representation, we develop multiple crowdsourcing approaches. Our core approach, at a high level, is a divide and conquer algorithm that applies a search space pruning strategy to efficiently identify if a dataset misses proper coverage for a given group. We provide a different theoretical analysis of our algorithm, including a tight upper bound on its performance which guarantees its near-optimality. Using this algorithm as the core, we propose multiple heuristics to reduce the coverage detection cost across different cases with multiple intersectional/non-intersectional groups. We demonstrate how the pre-trained predictors are not reliable and hence not sufficient for detecting representation bias in the data. Finally, we adjust our core algorithm to utilize existing models for predicting image group(s) to minimize the coverage identification cost. We conduct extensive experiments, including live experiments on Amazon Mechanical Turk to validate our problem and evaluate our algorithms' performance.

==> lemma1.tex <==

\noindent{\sc Lemma 1}
{\it
(Correctness) The \bc algorithm successfully identifies if a group $\gee$ is covered or not, i.e., if there are at least $\tau$ instances of $\gee$ in the data set $\dee$.
}
\vspace{2mm}


\begin{proof}
Each set query with a {\tt\small yes} answer contains at least one object belonging to the group $\gee$.
Using this, the algorithm maintains a lower bound $cnt$ on the $|\gee|$ in $\dee$. That is, $cnt\leq |\gee|$.
The algorithm returns {\tt\small true} when $cnt=\tau$.
When $cnt=\tau$, $\gee$ is covered, because $\tau = cnt \leq |\gee|$.
The algorithm returns false when the queue is empty and $cnt<\tau$.
For sets with {\tt\small yes} answers, the algorithm divides the set into two halves, unless the set size is $1$. As a result, when the queue is empty, all the set questions with {\tt\small yes} answers have had size $1$, otherwise, the queue would have not been empty.
Therefore, $|\gee| = cnt < \tau$, meaning that $\gee$ is uncovered.
\end{proof}

==> plots1.tex <==
\begin{figure*}[!tb]
\begin{minipage}[t]{0.63\linewidth}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/female.pdf}
        \caption{The relation between number of females in the dataset, the coverage threshold, and the number of questions}
        \label{fig:coverageX}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/cov.pdf}
        \caption{Varying coverage threshold}
        \label{fig:cov}
    \end{subfigure}
    % \hfill
    
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/subset.pdf}
        \caption{Varying subset size}
        \label{fig:subset}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/dataset.pdf}
        \caption{Varying dataset size}
        \label{fig:dataset}
    \end{subfigure}
    \caption{}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}[t]{0.32\linewidth}
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/nb_opt.pdf}
        \caption{Optimization for non-binary attribute vs. \bc}
        \label{fig:multi_bar}
    \end{subfigure}
    % \hfill
    
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/multi_opt.pdf}
        \caption{Optimization for multiple attributes vs. \bc }
        \label{fig:inter_bar}
    \end{subfigure}
    \caption{}
    \label{fig:opt}
\end{minipage}
\hrule
\begin{minipage}[t]{0.63\linewidth}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/nb_opt_dif_c.pdf}
        \caption{Non-binary attribute with $\mathbf{\sigma=3,4,5,6}$}
        \label{fig:nbOpt_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/multi_opt_dif_c.pdf}
        \caption{Optimization for 2 attributes $\mathbf{\sigma_1=2,\sigma_2=4}$ and 3 binary-values attributes}
        \label{fig:multiOpt_2}
    \end{subfigure}
    \caption{Non-binary and multiple attribute optimizations with varying number of attributes and cardinalities \bc}
\end{minipage}
\hfill\vline\hfill
\begin{minipage}[t]{0.32\linewidth}
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphs/amt.pdf}
        % \caption{Optimization for non-binary attribute vs. \bc}
        \label{fig:amt}
    \end{subfigure}
    % \hfill
    
    % \begin{tabular}{||P{0.60\linewidth} |P{0.15\linewidth}||}
    % \hline
    % \bf Dataset & \bf \#HITs \\ \hline
    %   FERET DB ({\small \tt females}=215, {\small \tt males}=1307)  & 74 \\ \hline
    %  FERET DB (unique) ({\small \tt females}=403, {\small \tt males}=591)  & 80 \\
    %  \hline
    % \end{tabular}
    \caption{The results of the experiments on Amazon Mechanical Turk on \bc }
    \label{fig:opt}
\end{minipage}
\end{figure*}



% \begin{figure*}[htbp]
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{graphs/female.pdf}
%         \caption{The relation between number of females in the dataset, the coverage threshold, and the number of questions}
%         \label{fig:coverageX}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{graphs/cov.pdf}
%         \caption{Varying coverage threshold}
%         \label{fig:cov}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{graphs/subset.pdf}
%         \caption{Varying subset size}
%         \label{fig:subset}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{graphs/dataset.pdf}
%         \caption{Varying dataset size}
%         \label{fig:dataset}
%     \end{subfigure}
%     \caption{Parameter analysis for \bc}
% \end{figure*}


% \begin{figure}[htbp]
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{graphs/nb_opt.pdf}
%         \caption{Optimization for non-binary attribute vs. \bc}
%         \label{fig:multi_bar}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.22\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{graphs/multi_opt.pdf}
%         \caption{Optimization for multiple attributes vs. \bc }
%         \label{fig:inter_bar}
%     \end{subfigure}
%     \caption{Comparison between the optimizations and \bc algorithm performance}
%     \label{fig:opt}
% \end{figure}
